Combining Weighted Total Variation and Deep Image Prior for natural and medical image restoration via ADMM

In the last decades, unsupervised deep learning based methods have caught researchers attention, since in many real applications, such as medical imaging, collecting a great amount of training examples is not always feasible. Moreover, the construction of a good training set is time consuming and hard because the selected data have to be enough representative for the task. In this paper, we focus on the Deep Image Prior (DIP) framework and we propose to combine it with a space-variant Total Variation regularizer with an automatic estimation of the local regularization parameters. Differently from other existing approaches, we solve the arising minimization problem via the flexible Alternating Direction Method of Multipliers (ADMM). Furthermore, we provide a specific implementation also for the standard isotropic Total Variation. The promising performances of the proposed approach, in terms of PSNR and SSIM values, are addressed through several experiments on simulated as well as real natural and medical corrupted images.

==> fig3.tex <==
\begin{figure*}[b!]
\centering
\includegraphics[scale=.38]{images/tomo/line_profile.png}
\caption{Line profiles by the starting \textit{tomo} grayscale test image, degraded with noise level $\sigma=30$, and DIP, DIPTV and ADMM DIP-TV reconstructions. The rows considered are the $90$-$th$ (top) and $370$-$th$ (bottom).}
\label{fig:lineprofile}
\end{figure*}

==> packages.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{bm} % bold greek letters
\usepackage{cases}
\usepackage{float}
\usepackage{mwe}
\usepackage{mathtools}
\usepackage{comment}
\usepackage{empheq}
\usepackage{booktabs}
\usepackage{textcomp}
\usepackage{algorithm,algorithmic}
\usepackage{array}
\usepackage{subfig}
\usepackage{url}
%\usepackage{caption}
\usepackage{multirow}
\usepackage{systeme}
%\usepackage{comment}
%\usepackage{float}
\usepackage{soul}



%\usepackage{amsmath}
%\newtheorem{theorem}{Theorem}
%\mathtoolsset{showonlyrefs}



%%Adding tikz

\usepackage{tikz}
\usetikzlibrary{positioning}
\usetikzlibrary{3d}
\usetikzlibrary{matrix}
\usetikzlibrary{decorations.text}
\usetikzlibrary{spy}

\makeatletter
\tikzoption{canvas is plane}[]{\@setOxy#1}
\def\@setOxy O(#1,#2,#3)x(#4,#5,#6)y(#7,#8,#9)%
{\def\tikz@plane@origin{\pgfpointxyz{#1}{#2}{#3}}%
	\def\tikz@plane@x{\pgfpointxyz{#4+#1}{#5+#2}{#6+#3}}%
	\def\tikz@plane@y{\pgfpointxyz{#7+#1}{#8+#2}{#9+#3}}%
	\tikz@canvas@is@plane
}
\makeatother
\tikzoption{canvas is xy plane at z}[]{%
	\def\tikz@plane@origin{\pgfpointxyz{0}{0}{#1}}%
	\def\tikz@plane@x{\pgfpointxyz{1}{0}{#1}}%
	\def\tikz@plane@y{\pgfpointxyz{0}{1}{#1}}%
	\tikz@canvas@is@plane
}
\makeatother



\usepackage[english]{babel}
\usepackage[utf8]{inputenc} % recommended for inputting accented characters
%\usepackage[T1]{fontenc} % recommended for languages different from English
\usepackage[bookmarks=false,hyperfootnotes=false]{hyperref}
\hypersetup{
			colorlinks=true,
			linkcolor=blue,
			anchorcolor=black,
			citecolor=green,
			urlcolor=blue
			}
\urlstyle{rm} % so it doesn't use a typewriter font for url's.

\usepackage{tipa}
 \expandafter\let\csname equation*\endcsname\relax
 \expandafter\let\csname endequation*\endcsname\relax
 
 

%\let\proof\relax
%\let\endproof\relax
%\usepackage{amsthm}

%

\newcommand{\CC}{\mathbb{C}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\NN}{\mathbb{N}}



% CALLIGRAPHIC LETTERS
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Zcal}{\mathcal{Z}}

% STANDING LETTERS
\newcommand{\Arm}{\mathrm{A}}
\newcommand{\Brm}{\mathrm{B}}
\newcommand{\Crm}{\mathrm{C}}
\newcommand{\Drm}{\mathrm{D}}
\newcommand{\Erm}{\mathrm{E}}
\newcommand{\Frm}{\mathrm{F}}
\newcommand{\Grm}{\mathrm{G}}
\newcommand{\Jrm}{\mathrm{J}}
\newcommand{\Krm}{\mathrm{K}}
\newcommand{\Irm}{\mathrm{I}}
\newcommand{\Hrm}{\mathrm{H}}
\newcommand{\Lrm}{\mathrm{L}}
\newcommand{\Mrm}{\mathrm{M}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\Orm}{\mathrm{O}}
\newcommand{\Prm}{\mathrm{P}}
\newcommand{\Qrm}{\mathrm{Q}}
\newcommand{\Rrm}{\mathrm{R}}
\newcommand{\Srm}{\mathrm{S}}
\newcommand{\Trm}{\mathrm{T}}
\newcommand{\Urm}{\mathrm{U}}
\newcommand{\Vrm}{\mathrm{V}}
\newcommand{\Xrm}{\mathrm{X}}
\newcommand{\Yrm}{\mathrm{Y}}
\newcommand{\Wrm}{\mathrm{W}}
\newcommand{\Zrm}{\mathrm{Z}}

% CAPITAL BOLD LETTERS
\newcommand{\Abold}{\mathbf{A}}
\newcommand{\Bbold}{\mathbf{B}}
\newcommand{\Cbold}{\mathbf{C}}
\newcommand{\Dbold}{\mathbf{D}}
\newcommand{\Ebold}{\mathbf{E}}
\newcommand{\Fbold}{\mathbf{F}}
\newcommand{\Gbold}{\mathbf{G}}
\newcommand{\Jbold}{\mathbf{J}}
\newcommand{\Kbold}{\mathbf{K}}
\newcommand{\Ibold}{\mathbf{I}}
\newcommand{\Hbold}{\mathbf{H}}
\newcommand{\Lbold}{\mathbf{L}}
\newcommand{\Mbold}{\mathbf{M}}
\newcommand{\Nbold}{\mathbf{N}}
\newcommand{\Obold}{\mathbf{O}}
\newcommand{\Pbold}{\mathbf{P}}
\newcommand{\Qbold}{\mathbf{Q}}
\newcommand{\Rbold}{\mathbf{R}}
\newcommand{\Sbold}{\mathbf{S}}
\newcommand{\Tbold}{\mathbf{T}}
\newcommand{\Ubold}{\mathbf{U}}
\newcommand{\Vbold}{\mathbf{V}}
\newcommand{\Xbold}{\mathbf{X}}
\newcommand{\Ybold}{\mathbf{Y}}
\newcommand{\Wbold}{\mathbf{W}}
\newcommand{\Zbold}{\mathbf{Z}}

% lowercase BOLD LETTERS
 \newcommand{\abold}{\mathbf{a}}
 \newcommand{\bbold}{\mathbf{b}}
 \newcommand{\cbold}{\mathbf{c}}
 \newcommand{\dbold}{\mathbf{d}}
 \newcommand{\ebold}{\mathbf{e}}
 \newcommand{\fbold}{\mathbf{f}}
 \newcommand{\gbold}{\mathbf{g}}
 \newcommand{\jbold}{\mathbf{j}}
 \newcommand{\kbold}{\mathbf{k}}
 \newcommand{\ibold}{\mathbf{i}}
 \newcommand{\hbold}{\mathbf{h}}
 \newcommand{\lbold}{\mathbf{l}}
 \newcommand{\mbold}{\mathbf{m}}
 \newcommand{\nbold}{\mathbf{n}}
 \newcommand{\obold}{\mathbf{o}}
 \newcommand{\pbold}{\mathbf{p}}
 \newcommand{\qbold}{\mathbf{q}}
 \newcommand{\rbold}{\mathbf{r}}
 \newcommand{\sbold}{\mathbf{s}}
 \newcommand{\tbold}{\mathbf{t}}
 \newcommand{\ubold}{\mathbf{u}}
 \newcommand{\vbold}{\mathbf{v}}
 \newcommand{\xbold}{\mathbf{x}}
 \newcommand{\ybold}{\mathbf{y}}
 \newcommand{\wbold}{\mathbf{w}}
\newcommand{\zbold}{\mathbf{z}}
%\newcommand{\abold}{{\bm{a}}}
%\newcommand{\bbold}{{\bm{b}}}
%\newcommand{\cbold}{{\bm{c}}}
%\newcommand{\dbold}{{\bm{d}}}
%\newcommand{\ebold}{{\bm{e}}}
%\newcommand{\fbold}{{\bm{f}}}
%\newcommand{\gbold}{{\bm{g}}}
%\newcommand{\jbold}{{\bm{j}}}
%\newcommand{\kbold}{{\bm{k}}}
%\newcommand{\ibold}{{\bm{i}}}
%\newcommand{\hbold}{{\bm{h}}}
%\newcommand{\lbold}{{\bm{l}}}
%\newcommand{\mbold}{{\bm{m}}}
%\newcommand{\nbold}{{\bm{n}}}
%\newcommand{\obold}{{\bm{o}}}
%\newcommand{\pbold}{{\bm{p}}}
%\newcommand{\qbold}{{\bm{q}}}
%\newcommand{\rbold}{{\bm{r}}}
%\newcommand{\sbold}{{\bm{s}}}
%\newcommand{\tbold}{{\bm{t}}}
%\newcommand{\ubold}{{\bm{u}}}
%\newcommand{\vbold}{{\bm{v}}}
%\newcommand{\xbold}{{\bm{x}}}
%\newcommand{\ybold}{{\bm{y}}}
%\newcommand{\wbold}{{\bm{w}}}
%\newcommand{\zbold}{{\bm{z}}}


\newcommand{\varphibold}{\bm{\varphi}}
\newcommand{\lambdabold}{\bm{\lambda}}
\newcommand{\Psibold}{\bm{\Psi}}
\DeclareMathOperator*{\argmin}{arg\,min}




